HR-pyPopStar: high wavelength-resolution stellar populations evolutionary synthesis model

We present the HR-pyPopStar model, which provides a complete set (in ages) of high resolution (HR) Spectral Energy Distributions of Single Stellar Populations. The model uses the most recent high wavelength-resolution theoretical atmosphere libraries for main sequence, post-AGB/planetary nebulae and Wolf-Rayet stars. The Spectral Energy Distributions are given for more than a hundred ages ranging from 0.1 Myr to 13.8 Gyr, at four different values of the metallicity (Z = 0.004, 0.008, 0.019 and 0.05), considering four different IMFs. The wavelength range goes from 91 to 24 000 {\AA} in linear steps {\delta}{\lambda} = 0.1 {\AA}, giving a theoretical resolving power R_{th,5000} ~ 50 000 at 5000 {\AA}. This is the main novelty of these spectra, unique for their age and wavelength ranges. The models include the ionising stellar populations that are relevant both at young (massive hot stars) as well as old (planetary nebulae) ages. We have tested the results with some examples of HR spectra recently observed with MEGARA at GTC. We highlight the importance of wavelength-resolution in reproducing and interpreting the observational data from the last and forthcoming generations of astronomical instruments operating at 8-10m class telescopes, with higher spectral resolution than their predecessors.

==> resto_indices.tex <==

% End of mnras_template.tex
\begin{table*}
\begin{center}
\caption{Definition of the lines that we have computed.}
\label{Table:9}
\begin{tabular}{cccccc}
\hline
Line name & $\rm \lambda_c$ & line bandpass & red bandpass & blue bandpass & Reference \\
    & (\AA) &   (\AA)   & (\AA) & (\AA)  \\
 BL1302 & 1302.0 & 1292.0 -- 1312.0 & 1270.0 -- 1290.0 & 1345.0 -- 1365.0 & F92 \\ 
 \ion{Si}{iv} 1397 & 1397.00 & 1387.0 -- 1407.0 & 1345.0 -- 1365.0 & 1475.0 -- 1495.0 & VID-GAR17 \\ 
  BL1425 & 1425.0 & 1415.0 -- 1435.0 & 1345.0 -- 1365.0 & 1475.0 -- 1495.0 & F92 \\ 
 \ion{Fe}{i} 1453  & 1453.00 & 1440.0 -- 1466.0 & 1345.0 -- 1365.0 & 1475.0 -- 1495.0 & VID-GAR17 \\
 \ion{C}{iv} 1540  & 1540.00 & 1530.0 -- 1550.0  & 1500.0 -- 1520.0 & 1577.0 -- 1597.0  & VID-GAR17 \\ %CIV in absorption\\ 
 \ion{C}{iv} 1548  & 1548.0 & 1540.0 -- 1560.0 & 1500.0 -- 1520.0  & 1577.0 -- 1597.0  & VID-GAR17 \\
 \ion{C}{iv} 1560  & 1560.00 & 1550.0 -- 1570.0  & 1500.0 -- 1520.0  & 1577.0 -- 1597.0  & VID-GAR17 \\ % CIV in emision\\
BL1617 & 1617.0 & 1604.0 -- 1630.0 & 1577.0 -- 1597.0 & 1685.0 -- 1705.0 & F92 \\ 
BL1664 & 1664.0 & 1651.0 -- 1677.0 & 1577.0 -- 1597.0 & 1685.0 -- 1705.0 & F92 \\ 
 \ion{Fe}{ii} 2402 & 2402.00 & 2382.0 -- 2422.0 & 2285.0 -- 2325.0 & 2432.0 -- 2458.0 & VID-GAR17 \\
 \ion{Fe}{ii} 2609 & 2609.00 & 2596.0 -- 2622.0 & 2562.0 -- 2588.0 & 2647.0 -- 2673.0 & VID-GAR17 \\ 
 \ion{Mg}{ii} 2800 & 2800.00 & 2784.0 -- 2814.0 & 2762.0 -- 2782.0  & 2818.0 -- 2838.0 & VID-GAR17 \\
 \ion{Mg}{i} 2852  & 2852.00 & 2839.0 -- 2865.0 & 2818.0 -- 2838.0  & 2906.0 -- 2936.0 & VID-GAR17 \\ 
 \ion{Fe}{i} 3000  & 3000.00 & 2965.0 -- 3025.0 & 2906.0 -- 2936.0 & 3031.0 -- 3051.0 & VID-GAR17 \\ 
 \ion{Ca}{i} 3934  & 3933.66 & 3926.6 -- 3940.6 & 3906.0 -- 3912.0  & 3948.0 -- 3954.0 & ROD-MER20 \\ % Ca I H line
 \ion{He}{i} 4026  & 4026.00 & 4020.0 -- 4031.0 & 4012.0 -- 4020.0 & 4158.0 -- 4169.0 & GON05 \\
 \ion{Fe}{i} 4046  & 4045.81 & 4044.8 -- 4046.8  & 4036.0 -- 4041.0  & 4052.0 -- 4057.0 & ROD-MER20 \\ 
  $H_\delta$       & 4101.73 & 4092.0 -- 4112.0 & 4012.0 -- 4020.0 & 4158.0 -- 4169.0 & GON05 \\ 
  $H_\gamma$       & 4340.47 & 4330.0 -- 4350.0 & 4262.0 -- 4270.0 & 4445.0 -- 4453.0 & GON05 \\ 
 %\ion{He}{i} 4471  & 4471.00 & 4464 --4478.0 &  &  \\
 \ion{Mg}{i} 4480  & 4481.13 & 4480.8 -- 4481.9 & 4473.0 -- 4478.0 & 4484.0 -- 4489.0 & ROD-MER20 \\
  $H_\beta$        & 4861.35 & 4852.0 -- 4872.0 & 4770.0 -- 4782.0 & 4942.0 -- 4954.0 & GON05 \\ 
 \ion{He}{i} 5876  & 5876.00 & 5871.0 -- 5880.0 & 5835.0 -- 5845.0 & 5904.0 -- 5912.0 & GON05 \\
  $H_\alpha$       & 6562.79 & 6553.0 -- 6573.0 & 6506.0 -- 6514.0 & 6612.0 -- 6620.0 & GON05 \\
% Pa1               & 8467.27 & 8461.0 -- 8474.0 &  & 8474.0 -- 8484.0  & GV20 \\
 Pa2               & 8598.40 & 8577.0 -- 8619.0 & 8563.0 -- 8577.0 & 8619.0 -- 8642.0 & GV20 \\
 Pa3               & 8750.47 & 8730.0 -- 8772.0 & 8700.0 -- 8725.0 & 8776.0 -- 8792.0  & GV20 \\
 CaT1              & 8498.03 & 8482.0 -- 8512.0 & 8450.0 -- 8460.0 & 8565.5 -- 8575.0 & GV20 \\
 CaT2              & 8542.09 & 8531.0 -- 8554.0 & 8450.0 -- 8460.0 &  8565.5 -- 8575.0 & GV20 \\
 CaT3              & 8662.14 & 8650.0 -- 8673.0 & 8619.5 -- 8642.5 & 8700.5 -- 8710.0 & GV20 \\
 \ion{Mg}{i} 8807  & 8807.00 & 8802.5 -- 8811.0 & 8781.0 -- 8789.0 & 8831.0 -- 8835.5 & CEN09 \\
\end{tabular}
\end{center}
\footnotesize{References. F92: \citet{Fanelli+1992}, CEN01: \citet{cen01}, GON05: \citet{Gonzalez+2005}, CEN09: \citet{cen09}, VID-GAR17: \citet{vidal-garcia2017}, ROD-MER20: \citet{rodriguez-merino20},and GV20: \citet{gv20}.}
\end{table*}


\begin{table}
\begin{center}
\caption{Equivalent width of the lines defined in Table \ref{Table:9}.}
\label{Table:10}
\begin{turn}{90}
\begin{tabular}{cccccccccccccc}
\hline
log(age) & BL1302  & Si IV 1397 & BL1425 & Fe I 1453 & C IV 1540 & C IV 1550 & C IV 1560 & BL1617 & BL 1664 & Fe II 2402 & Fe II 2609 & Mg II 2800 & Mg I 2852\\
%& Mg I 2800 & Ca I 3934 & Fe I 4046 & Mg I 4480 & $\rm H_{\alpha}$ & Pa2 & Pa3 & CaT
dex  & (\AA) &  (\AA)& (\AA)   &   (\AA)   & (\AA) & (\AA) & (\AA) & (\AA)& (\AA)& (\AA)& (\AA) & (\AA) \\
\hline
5.00 & 0.002 & 0.081 & 0.034 & 0.034 & 6.402 & -0.023 &  -1.670 & 0.048 & 0.026 & 0.297 & 0.298 & 0.308 & 0.069 \\
5.48 & 0.002 & 0.088 & 0.038 & 0.038 & 6.689 & 0.001 & -1.675 & 0.052 & 0.028 & 0.293 & 0.294 & 0.306 & 0.062 \\
5.70 & 0.003 & 0.089 & 0.039 & 0.039 & 6.938 & 0.039 & -1.661 & 0.055 & 0.029 & 0.300 & 0.300 & 0.315 & 0.075 \\
5.85 & 0.004 & 0.084 & 0.038 & 0.037 & 6.920 & 0.012 & -1.663 & 0.065 & 0.034 & 0.310 & 0.310 & 0.329 & 0.106 \\
6.00 & 0.003 & 0.096 & 0.045 & 0.048 & 7.527 & -0.296 & -1.789 & 0.070 & 0.037 & 0.314 & 0.314 & 0.318 & 0.068 \\
6.10 & 0.002 & 0.092 & 0.045 & 0.049 & 8.245 & -0.412 & -2.077 & 0.071 & 0.039 & 0.286 & 0.286 & 0.308 & 0.084 \\
6.18 & 0.002 & 0.080 & 0.041 & 0.045 & 8.717 & -0.087 & -2.132 & 0.089 & 0.047 & 0.285 & 0.285 & 0.325 & 0.136 \\
6.24 & 0.000 & 0.093 & 0.051 & 0.055 & 9.437 & 0.484 & -2.050 & 0.095 & 0.050 & 0.299 & 0.299 & 0.329 & 0.121 \\
6.30 & -0.001 & 0.082 & 0.049 & 0.050 & 9.841 & 1.091 & -1.977 & 0.096 & 0.051 & 0.260 & 0.260 & 0.353 & 0.239 \\
%6.35 & 0.000 & 0.079 & 0.046 & 0.045 & 9.977 & 1.535 & -1.864 & 0.110 & 0.054 & 0.252 & 0.252 & 0.366 & 0.336 \\
%6.40 & 0.006 & 0.109 & 0.062 & 0.050 & 10.414 & 2.120 & -1.665 & 0.122 & 0.057 & 0.159 & 0.159 & 0.414 & 0.286 \\
%6.44 & 0.015 & 0.144 & 0.078 & 0.055 & 10.512 & 2.686 & -1.238 & 0.132 & 0.059 & 0.090 & 0.090 & 0.475 & 0.236 \\
%6.48 & 0.022 & 0.176 & 0.094 & 0.066 & 10.520 & 3.114 & -0.883 & 0.126 & 0.056 & 0.040 & 0.040 & 0.511 & 0.172 \\
%6.51 & 0.035 & 0.207 & 0.102 & 0.064 & 10.137 & 2.351 & -1.405 & 0.113 & 0.045 & 0.019 & 0.019 & 0.564 & 0.218 \\
%6.54 & 0.058 & 0.263 & 0.117 & 0.052 & 9.523 & 1.704 & -1.541 & 0.102 & 0.040 & 0.098 & 0.098 & 0.745 & 0.138 \\
%6.57 & 0.073 & 0.273 & 0.114 & 0.032 & 9.228 & 1.418 & -1.560 & 0.099 & 0.035 & 0.220 & 0.220 & 0.858 & 0.111 \\
%6.60 & 0.080 & 0.302 & 0.125 & 0.023 & 9.152 & 1.988 & -0.818 & 0.101 & 0.034 & 0.460 & 0.460 & 1.018 & -0.021 \\
%6.63 & 0.077 & 0.327 & 0.129 & 0.024 & 9.123 & 1.922 & -0.825 & 0.104 & 0.035 & 0.608 & 0.608 & 1.058 & -0.047 \\
%6.65 & 0.076 & 0.354 & 0.133 & 0.031 & 9.279 & 1.961 & -0.937 & 0.102 & 0.036 & 0.456 & 0.456 & 1.001 & -0.053 \\
%6.68 & 0.081 & 0.386 & 0.145 & 0.041 & 9.523 & 2.974 & -0.250 & 0.107 & 0.038 & 0.249 & 0.249 & 0.998 & -0.017 \\
%6.70 & 0.079 & 0.388 & 0.153 & 0.051 & 9.575 & 3.619 & 0.244 & 0.093 & 0.034 & 0.202 & 0.202 & 0.989 & 0.010 \\
%6.72 & 0.085 & 0.413 & 0.157 & 0.056 & 9.453 & 3.923 & 0.432 & 0.120 & 0.044 & 0.142 & 0.142 & 1.028 & 0.021 \\
%6.74 & 0.086 & 0.378 & 0.144 & 0.032 & 9.504 & 4.549 & 1.122 & 0.089 & 0.036 & 0.331 & 0.331 & 1.037 & 0.060 \\
%6.76 & 0.118 & 0.425 & 0.140 & 0.010 & 8.855 & 4.142 & 1.298 & 0.088 & 0.041 & 0.155 & 0.155 & 0.997 & 0.051 \\
%6.78 & 0.124 & 0.399 & 0.133 & 0.004 & 8.426 & 3.974 & 1.482 & 0.090 & 0.053 & 0.396 & 0.396 & 0.978 & 0.048 \\
%6.81 & 0.116 & 0.419 & 0.140 & 0.014 & 8.819 & 4.301 & 1.680 & 0.079 & 0.044 & 0.277 & 0.277 & 1.261 & 0.047 \\
%6.85 & 0.116 & 0.454 & 0.145 & 0.013 & 8.931 & 4.688 & 2.376 & 0.078 & 0.042 & 0.187 & 0.187 & 1.655 & 0.055 \\
%6.86 & 0.119 & 0.447 & 0.143 & 0.013 & 8.755 & 4.639 & 2.355 & 0.065 & 0.034 & 0.177 & 0.177 & 1.597 & 0.056 \\
%6.88 & 0.122 & 0.450 & 0.142 & 0.005 & 8.602 & 4.726 & 1.564 & 0.058 & 0.032 & -0.126 & -0.126 & 1.225 & 0.060 \\
%6.89 & 0.122 & 0.457 & 0.142 & 0.001 & 8.662 & 4.846 & 1.230 & 0.056 & 0.031 & -0.243 & -0.243 & 1.145 & 0.061 \\
%6.90 & 0.122 & 0.457 & 0.142 & 0.000 & 8.629 & 4.831 & 0.995 & 0.053 & 0.031 & -0.290 & -0.290 & 1.063 & 0.061 \\
%6.92 & 0.121 & 0.453 & 0.140 & -0.002 & 8.630 & 4.800 & 0.593 & 0.050 & 0.030 & -0.337 & -0.337 & 0.962 & 0.058 \\
%6.93 & 0.117 & 0.461 & 0.141 & -0.003 & 8.878 & 4.935 & 0.476 & 0.044 & 0.028 & -0.377 & -0.337 & 0.976 & 0.057 \\
%6.94 & 0.120 & 0.460 & 0.140 & -0.007 & 8.703 & 4.955 & 0.464 & 0.040 & 0.027 & -0.389 & -0.389 & 0.970 & 0.061 \\
%6.95 & 0.122 & 0.461 & 0.140 & -0.009 & 8.574 & 5.024 & 0.522 & 0.035 & 0.025 & -0.390 & -0.390 & 0.977 & 0.064 \\
%6.97 & 0.127 & 0.458 & 0.139 & -0.013 & 8.310 & 5.032 & 0.612 & 0.032 & 0.024 & -0.382 & -0.382 & 0.986 & 0.069 \\
%6.98 & 0.130 & 0.456 & 0.138 & -0.015 & 8.141 & 5.020 & 0.622 & 0.026 & 0.023 & -0.374 & -0.374 & 0.986 & 0.072 \\
%6.99 & 0.135 & 0.456 & 0.138 & -0.020 & 7.916 & 5.045 & 0.639 & 0.021 & 0.021 & -0.372 & -0.372 & 1.006 & 0.077 \\
%7.00 & 0.139 & 0.454 & 0.137 & -0.023 & 7.724 & 5.055 & 0.656 & 0.011 & 0.017 & -0.370 & -0.370 & 1.007 & 0.080 \\
%7.04 & 0.149 & 0.442 & 0.133 & -0.032 & 7.172 & 4.883 & 0.823 & 0.000 & 0.014 & -0.278 & -0.278 & 1.039 & 0.086 \\
%7.08 & 0.159 & 0.424 & 0.127 & -0.041 & 6.540 & 4.691 & 1.023 & -0.006 & 0.014 & -0.128 & -0.128 & 1.126 & 0.091 \\
%7.11 & 0.163 & 0.415 & 0.124 & -0.046 & 6.283 & 4.582 & 1.191 & -0.011 & 0.009 & -0.022 & -0.022 & 1.219 & 0.094 \\ 
%7.15 & 0.177 & 0.393 & 0.118 & -0.054 & 5.642 & 4.281 & 1.093 & -0.012 & 0.008 & 0.023 & 0.023 & 1.071 & 0.098 \\
%7.18 & 0.188 & 0.374 & 0.113 & -0.057 & 5.156 & 4.019 & 1.012 & -0.011 & 0.008 & 0.101 & 0.101 & 0.999 & 0.100 \\
%7.20 & 0.200 & 0.353 & 0.107 & -0.060 & 4.591 & 3.723 & 0.949 & -0.007 & 0.010 & 0.194 & 0.194 & 0.917 & 0.103 \\
\hline
\end{tabular}
\end{turn}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{Continuation of table 10 }
\label{Table:10b}
\begin{turn}{90}
\begin{tabular}{cccccccccccccccc}
\hline
Fe I 3000 & Ca I 3934 & He I 4026 & Fe I 4046 & $\rm H_{\delta}$ & $\rm H_{\gamma}$ & Mg I 4480 & $\rm H_{\beta}$ & He I 5876 & $\rm H_{\alpha}$ & Pa2 & Pa3 & CaT1 & CaT2 & CaT3 & Mg I 8807\\ 
(\AA) & (\AA) &  (\AA)& (\AA)  & (\AA) &   (\AA)   & (\AA) & (\AA) & (\AA) & (\AA)& (\AA)& (\AA)& (\AA) & (\AA) & (\AA) \\
\hline
0.150 & 0.024 & 0.591 & 0.001 & 2.538 & 2.394 & 0.068 & 0.810 & 6.402 & -0.023 & -1.670 & 0.297 & 0.298 & 0.308 & 0.069 & 0.150 \\
0.135 & 0.029 & 0.592 & 0.000 & 2.532 & 2.384 & 0.068 & 2.251 & 0.339 & 1.397 & 0.373 & 0.834 & 0.091 & 0.201 & 0.459 & -0.019 \\
0.159 & 0.028 & 0.599 & 0.000 & 2.520 & 2.375 & 0.068 & 2.247 & 0.342 & 1.398 & 0.388 & 0.857 & 0.096 & 0.209 & 0.474 & -0.019 \\
0.233 & 0.020 & 0.602 & 0.001 & 2.481 & 2.352 & 0.068 & 2.226 & 0.329 & 1.381 & 0.394 & 0.863 & 0.099 & 0.213 & 0.481 & -0.018 \\
0.190 & 0.030 & 0.605 & 0.000 & 2.499 & 2.373 & 0.068 & 2.285 & 0.366 & 1.491 & 0.417 & 0.894 & 0.106 & 0.227 & 0.510 & -0.018 \\
0.236 & 0.026 & 0.608 & 0.000 & 2.477 & 2.343 & 0.067 & 2.282 & 0.389 & 1.526 & 0.453 & 0.939 & 0.108. & 0.251 & 0.546 & -0.017 \\
0.320 & 0.017 & 0.620 & 0.000 & 2.467 & 2.320 & 0.068 & 2.274 & 0.434 & 1.532 & 0.486 & 0.986 & 0.109 & 0.270 & 0.575 & -0.017 \\
0.284 & 0.028 & 0.620 & 0.000 & 2.446 & 2.277 & 0.068 & 2.275 & 0.508 & 1.588 & 0.545 & 1.048 & 0.102 & 0.313 & 0.630 & -0.016 \\
0.539 & 0.019 & 0.624 & 0.000 & 2.409 & 2.224 & 0.069 & 2.260 & 0.583 & 1.622 & 0.621 & 1.120 & 0.099 & 0.368 & 0.690 & -0.016 \\
0.763 & 0.015 & 0.618 & 0.000 & 2.344 & 2.142 & 0.070 & 2.195 & 0.597 & 1.567 & 0.697 & 1.186 & 0.125 & 0.428 & 0.757 & -0.015 \\
%0.635 & 0.018 & 0.636 & -0.001 & 2.382 & 2.152 & 0.077 & 2.255 & 0.663 & 1.685 & 0.839 & 1.333 & 0.238 & 0.522 & 0.896 & -0.016 \\
%0.561 & 0.014 & 0.640 & -0.001 & 2.352 & 2.145 & 0.085 & 2.276 & 0.724 & 1.782 & 1.012 & 1.487 & 0.376 & 0.647 & 1.062 & -0.016 \\
%0.443 & 0.016 & 0.634 & 0.003 & 2.279 & 2.065 & 0.089 & 2.156 & 0.727 & 1.451 & 1.108 & 1.546 & 0.462 & 0.722 & 1.149 & -0.016 \\
%0.411 & -0.015 & 0.635 & 0.001 & 2.241 & 2.077 & 0.101 & 2.092 & 0.826 & 1.270 & 1.270 & 1.671 & 0.571 & 0.826 & 1.279 & -0.014 \\
%0.344 & -0.021 & 0.659 & -0.004 & 2.275 & 2.112 & 0.138 & 2.110 & 0.914 & 1.299 & 1.531 & 1.868 & 0.807 & 1.034 & 1.512 & -0.013 \\
%0.354 & -0.019 & 0.671 & -0.006 & 2.300 & 2.113 & 0.167 & 2.138 & 0.926 & 1.422 & 1.665 & 1.969 & 0.926 & 1.162 & 1.632 & -0.012 \\
%0.381 & 0.014 & 0.689 & -0.005 & 2.323 & 2.043 & 0.200 & 2.136 & 0.940 & 1.394 & 1.819 & 2.083 & 1.072 & 1.311 & 1.784 & -0.014 \\
%0.385 & 0.028 & 0.703 & -0.005 & 2.385 & 2.037 & 0.220 & 2.171 & 0.945 & 1.347 & 1.872 & 2.166 & 1.104 & 1.352 & 1.844 & -0.016 \\
%0.356 & 0.024 & 0.720 & -0.005 & 2.526 & 2.167 & 0.210 & 2.266 & 0.933 & 1.331 & 1.807 & 2.188 & 1.011 & 1.264 & 1.800 & -0.018 \\
%0.264 & 0.017 & 0.734 & -0.001 & 2.645 & 2.279 & 0.199 & 2.336 & 0.907 & 1.207 & 1.742 & 2.199 & 0.932 & 1.193 & 1.769 & -0.025 \\
%0.205 & 0.014 & 0.747 & 0.000 & 2.669 & 2.294 & 0.195 & 2.309 & 0.832 & 0.741 & 1.728 & 2.205 & 0.895 & 1.175 & 1.767 & -0.029 \\
%0.191 & 0.020 & 0.753 & 0.008 & 2.694 & 2.294 & 0.192 & 2.285 & 0.861 & 0.669 & 1.728 & 2.218 & 0.877 & 1.165 & 1.781 & -0.033 \\
%0.399 & 0.006 & 0.764 & -0.002 & 2.637 & 2.275 & 0.207 & 2.316 & 0.716 & 0.591 & 1.805 & 2.286 & 0.956 & 1.255 & 1.850 & -0.029 \\
%0.366 & 0.258 & 0.786 & 0.047 & 2.843 & 2.575 & 0.193 & 2.855 & 0.695 & 2.222 & 1.298 & 1.705 & 1.637 & 3.394 & 3.415 & 0.342 \\
%0.305 & 0.327 & 0.778 & 0.042 & 3.239 & 2.926 & 0.217 & 3.193 & 0.617 & 2.445 & 1.482 & 2.019 & 1.636 & 3.321 & 3.463 & 0.321 \\
%0.024 & 0.407 & 0.615 & 0.048 & 3.569 & 3.411 & 0.227 & 3.646 & 0.436 & 3.033 & 1.680 & 2.270 & 1.723 & 3.261 & 3.480 & 0.312 \\
%0.115 & 2.469 & 0.589 & 0.110 & 5.034 & 5.106 & 0.264 & 5.157 & 0.330 & 4.057 & 2.376 & 3.334 & 2.143 & 3.839 & 4.238 & 0.344 \\
%0.133 & 2.960 & 0.607 & 0.124 & 5.253 & 5.314 & 0.265 & 5.308 & 0.319 & 4.102 & 2.355 & 3.358 & 2.160 & 3.938 & 4.311 & 0.356 \\
%0.223 & 3.122 & 0.705 & 0.190 & 4.209 & 4.177 & 0.243 & 4.442 & 0.287 & 3.508 & 1.564 & 2.162 & 2.206 & 4.625 & 4.466 & 0.448 \\
%0.286 & 2.535 & 0.744 & 0.220 & 3.706 & 3.591 & 0.229 & 4.012 & 0.264 & 3.138 & 1.230 & 1.658 & 2.252 & 4.975 & 4.583 & 0.493 \\ 
%0.351 & 1.871 & 0.785 & 0.222 & 3.436 & 3.242 & 0.215 & 3.709 & 0.270 & 2.796 & 0.995 & 1.334 & 2.234 & 5.144 & 4.625 & 0.546 \\
%0.429 & 0.820 & 0.842 & 0.244 & 2.932 & 2.811 & 0.191 & 3.326 & 0.260 & 2.272 & 0.593 & 0.878 & 2.350 & 5.749 & 5.019 & 0.720 \\
%0.362 & 0.508 & 0.923 & 0.240 & 2.996 & 2.752 & 0.179 & 3.250 & 0.327 & 1.978 & 0.476 & 0.813 & 1.936 & 5.293 & 4.619 & 0.886 \\
%0.312 & 0.315 & 0.980 & 0.190 & 3.341 & 2.860 & 0.175 & 3.281 & 0.399 & 1.863 & 0.464 & 0.834 & 1.618 & 4.918 & 4.326 & 0.958 \\
%0.298 & 0.166 & 0.996 & 0.118 & 3.702 & 3.040 & 0.179 & 3.343 & 0.490 & 1.828 & 0.522 & 0.883 & 1.332 & 4.520 & 4.035 & 0.958 \\
%0.317 & 0.137 & 0.981 & 0.088 & 3.795 & 3.216 & 0.185 & 3.504 & 0.570 & 1.975 & 0.612 & 1.011 & 1.381 & 4.470 & 4.105 & 0.890 \\
%0.332 & 0.161 & 0.978 & 0.093 & 3.778 & 3.222 & 0.187 & 3.517 & 0.556 & 2.007 & 0.622 & 1.015 & 1.440 & 4.540 & 4.165 & 0.874 \\
%0.357 & 0.202 & 0.971 & 0.098 & 3.772 & 3.234 & 0.191 & 3.542 & 0.541 & 2.060 & 0.639 & 1.020 & 1.528 & 4.654 & 4.260 & 0.848 \\
%0.370 & 0.237 & 0.970 & 0.099 & 3.800 & 3.264 & 0.194 & 3.579 & 0.536 & 2.110 & 0.656 & 1.035 & 1.567 & 4.698 & 4.304 & 0.831 \\ 
%0.382 & 0.727 & 0.946 & 0.107 & 4.031 & 3.538 & 0.210 & 3.865 & 0.513 & 2.380 & 0.823 & 1.221 & 1.575 & 4.604 & 4.290 & 0.784 \\
%0.375 & 1.324 & 0.906 & 0.105 & 4.548 & 4.127 & 0.229 & 4.337 & 0.495 & 2.618 & 1.023 & 1.505 & 1.553 & 4.477 & 4.288 & 0.775 \\ 
%0.354 & 1.161 & 0.873 & 0.083 & 4.681 & 4.322 & 0.238 & 4.509 & 0.512 & 2.791 & 1.191 & 1.737 & 1.512 & 4.223 & 4.179 & 0.725 \\ 
%0.411 & 0.882 & 0.950 & 0.071 & 4.676 & 4.245 & 0.228 & 4.421 & 0.564 & 2.607 & 1.093 & 1.667 & 1.391 & 4.100 & 4.077 & 0.726 \\
%0.432 & 0.807 & 0.977 & 0.075 & 4.648 & 4.183 & 0.225 & 4.369 & 0.556 & 2.504 & 1.012 & 1.559 & 1.376 & 4.167 & 4.095 & 0.751 \\
%0.448 & 0.713 & 0.999 & 0.077 & 4.575 & 4.089 & 0.221 & 4.300 & 0.543 & 2.410 & 0.949 & 1.469 & 1.370 & 4.230 & 4.118 & 0.772 \\
\hline
\end{tabular}
\end{turn}
\end{center}
\end{table}

\begin{figure*}
    \centering
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_a.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_b.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_c.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_d.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_e.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_f.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_g.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10a_h.pdf}
    \caption{Comparison of the time evolution of the equivalent width of the selected lines between pyPopStar using CHA IMF, MILES using CHA IMF, GON05 using CHA IMF, CB2018 parsec, CB2018 pmiles and CB2018 smiles.}
    \label{Fig:10a}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_a.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_b.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_c.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_d.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_e.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_f.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_g.pdf}
    \includegraphics[width=0.33\textwidth]{figpdf/millan_fig10b_h.pdf}
    \caption{Comparison of the time evolution of the equivalent width of the selected lines between pyPopStar using SAL IMF, MILES using SAL IMF, GON05 using SAL IMF, Ma20 emp, Ma20 theo and UVBLUE.}
    \label{Fig:10b}
\end{figure*}

%\textcolor{red}{MER:Quitaria todo este parrafo
%There are several effects to be considered in the computation of the stellar isochrones: stellar mass loss, pre-main sequence (PMS) phase, overshooting and stellar rotation:
%\begin{enumerate}
%\item The stellar mass loss determines, for the youngest populations and  closely related to the abundance, the evolution of massive stars and their transition to the WR phase. Also, the mass loss is an important factor to determine the stellar mass that remains in the post-AGB and planetary nebulae stars at intermediate-old ages.  
%\textcolor{cyan}{\bf{Dejo un párrafo que había comentado ligeramente modificado}}
%\textcolor{cyan}{
%\item Some of our models at the youngest ages contain stars in the Pre-Main Sequence, PMS, phase. These stars are still surrounded by the molecular cloud where they form, so some dust attenuation of their light is expected. However, at the early ages, even if a significant fraction of low-mass stars are in the PMS, the most massive ones dominate the spectrum. As a result, the effect of this dust attenuation of the spectra would not be relevant for the final result. Nevertheless, the isochrones we use have not included any dust.
%}
%\item Given that our aim is to model the maximum age range, some of the %models lay in ages where some of the stars are still in the Pre-Main %Sequence, PMS, phase. These stars may be embedded inside the molecular %clouds where they were formed, what could diminish their flux. We have not %considered the impact of this effect that will be explored in future %works.
%{\bf mcs: Cambiaría la frase ya que te metes en berenjenales no deseados: no puedes asegurar que las estrellas de alta masa no estén tambien embebidas en la nube molecular osea, tambien afectadas por dust atenuation!!... Formalmente PARSEC no considera que las estrellas esten embebidas o no, el polvo no existe en esos modelos solo dice que acreta, pero no dice "de donde".... ()}
%\item The convective core overshooting is the insertion of the convective zone into the radiative zone. It is known that the overshooting is a relevant process for the stellar evolution mainly for the massive and intermediate mass stars. The overshooting mixes the inner layers with the outer ones, bringing fresh fuel for the core of the star, enhancing their lifetime.  Furthermore, this process modifies the element abundance of the stellar atmosphere. 
%Y:?? como queda esto? se ha incluido en las isocronas? como afecta?
%Iker: No hemos cambiado las isocronas para nada. Cuando los de PARSEC nos pasen isocronas que contengan post-AGB y PNe las cambiaremos por esas en las que te da la abundancia superficial de H,He,C,N,O.
% Yo diria que el overshooting ya estaba incluido en la isocronas viejas, no deberia ser un issue ahora...
%mcs: si, overshooting siempre ha estado incluido para masivas. El problema entre los dos no es el overshotting en si, sino Como definirlo": es un criterio de "acelaracion" con lo cual la cantidad de overshoting se puede definir por acelaricón o por velocidad: donde cesa el "empuje" y donde "para". Segun el criterio el nucleo convectivo es mas grande o mas pequeño y es el lio, uno de ellos, entre padova y Ginebra
%\end{enumerate}}

%\begin{table}
%	\begin{center}
%	\caption{Chemical abundances of the WR atmosphere models.}
%\label{Table:4}
%	\begin{tabular}{|l|l|l|l|l|l|}
%\hline
%Name & $Z$ & $X_{\rm H}$ & $X_{\rm He}$ & $X_{\rm C}$ & $X_{\rm N}$\\
%\hline
%$\rm WNL-H20_{SMC}$ & 0.0024 & 0.2 & 0.798 & $2.5 \ %10^{-5}$ & $1.5 \ 10^{-3}$ \\
%& & & & & \\
%$\rm WNL-H20_{LMC}$ & 0.008 & 0.2 & 0.795 & $7 \ 10^{-5}$  & $4 \ 10^{-3}$ \\
%$\rm WC_{LMC}$ & 0.008 & 0.0 & 0.55 & 0.4 & 0.0 \\
%& & & & & \\
%$\rm WNL-H20_{MW}$ & 0.017 & 0.2 & 0.78 & $10^{-4}$ %& 0.015 \\
%$\rm WC_{MW}$ & 0.017 & 0.0 & 0.55 & 0.4 & 0.0 \\
%\hline
%		\end{tabular}
%	\end{center}
%\end{table}
%Finally, we have computed equivalent width and spectral indices in the pyPopstar SSPs to demonstrate the utility of our high spectral resolution models for tracing stellar populations through their contribution to the absorption lines. \pc{Table~\ref{Table:9} lists the indices and lines measured in our models}. Table \ref{Table:10} shows the results of all computed lines for the first youngest SSPs, assuming the CHA IMF and $Z_{\sun}$. 

%, we have selected some lines to represent the time evolution of equivalent widths and indices and to compare them with results from other models found in the literature. The selected indices, covering from UV to the near IR, are Mg I 2800, Ca I 3934, Fe I 4046, Mg I 4480, $\rm H_{\alpha}$, CaT, Pa2 and Pa3. The time evolution of the rest of the computed lines is available in the electronic version only. We have compared our CHA IMF models with the ones by V16, GON05 and CB2018; and our SAL IMF models with those by UVBLUE Maraston, M20 and V16.

%\textcolor{cyan}{\bf{Si estamos poniendo la misma definición del índice yo no esperaría diferencias apreciables en los valores debido a la alta resolución. Si se ponen las mismas ventanas las diferencias se deben - fundamentalmente - a otras entradas, como los modelos, o las isocronas. Digo fundamentalmente porque si se tienen modelos de alta resolución en general vamos a tener más en líneas y menos en continuo - al final la energía es la misma - por lo que yo siempre esperaría que a igualdad de definición y de otras cosas, nuestros modelos estuvieran un poco por encima al comparar con los de baja resolución. Pero las diferencias que se ven son grandes. La importancia de la alta resolución no es para medir mejor o peor el índice, sino para ser capaces de definir nuevos índices que estén de-contaminados de otras líneas diferentes a las que se quiere medir, y que pueden venir de poblaciones estelares muy distintas. Por ejemplo en el caso del CaT cuando se mide a baja resolución se están metiendo líneas de Fe que desaparecen cuando medimos a alta resolución. Las diferencias van a deberse a una diferente definición de las ventanas de continuo y, sobre todo, de la línea. }}

%\pc{[at least in terms of lick-like indices, changes in resolution will change the measured values. so i don't think it makes sense to compare among models unless we bring all of them to the same resolution. and different indices react differently to resolution. i will try to find in literature examples of how much change we expect from just changing the resolution.]}

%Firstly, we will compare the Mg II 2800. It can be observed that its evolution in pyPopStar is very similar to UVBLUE, but very different to MILES irrespective of the IMF. This difference may be caused by the discrepancies between the computation of the Mg lines in the UV range in theoretical stellar libraries and observed in empirical stellar libraries.
%UVBLUE no se ve en Mg II. Iker: es la linea morada que está pegada a la linea de pyPopStar, por eso no se ve
%\textcolor{cyan}{\bf{Si nos metemos a comparar hay que desentrañar de dónde vienen las diferencias. Pueden venir de los modelos de atmósferas, de una diferente definición del índice, de la introducción o no del continuo nebular, sobre todo para líneas UV y visibles, etc. Y tenemos que estar seguros. Si es una región espectral muy poblada de líneas, podría ser que la alta resolución aumentara mucho la intensidad de líneas frente al continuo - que va a bajar al conservar la energía - y eso podría darnos valores más altos del índice. a mi este tema me parece de lo más interesante para hacer un paper dedicado, la verdad.}}

%Secondly, the Ca I 3934 line of pyPopStar in both IMFs is very similar to all the rest of the models at young and intermediate age. However, differences begin to appear at late ages. On one hand, when we compare the EW of Ca I 3934 with other models that use theoretical stellar spectra, we see that the results are similar. On the other hand, pyPopStar models and empirical models differ significantly. This disagreement between pyPopStar and the empirical may be caused by the difference in the stellar libraries. \textcolor{cyan}{\bf{No sé si pueda deberse a un aumento del continuo nebular en esa región del espectro, que venga de las nebulosas planetarias. Hay que plotear el continuo en esas longitudes de onda de los modelos comparados, para ver si se debe a eso}}

%Another intare Fe I 4046 and Mg I 4480, these very narrow and weak lines exemplify the difference between HR spectra and SSP with lower resolutions. In these case, the EW of pyPopStar models are bigger than the rest, except from MARUV. The reason behind this discrepancy is that in the models whose resolution is comparable to the range of the line definition the EW of these line may be underestimated. This lines are very illustrative of the potential of our models to reproduce and use weak absorption lines in the analysis. \pc{[detecting weak absorption lines at the level of the models will not be so useful in extragalactic studies because what limits that is the velocity dispersion of the system, which will wash out the thin lines even if the observation is at high resolution]}\textcolor{cyan}{\bf{hay que mejorar y cuantificar este argumento. como digo hay que estar muy seguro en cada caso a qué se debe la diferencia y puede ayudar pintar el espectro de los diferentes modelos en el intervalo en cuestión. Se puede normalizar ya que si estamos midiendo anchuras equivalente no importa el nivel del continuo en términos absolutos. Lo mismo para los párrafos siguientes. Nos tenemos que currar más los argumentos si vamos a poner la comparación.}}

%Concerning $\rm H_{\alpha}$ line, pyPopStar models are very similar to all of the SSP models except CB2018 \pc{[from what is shown in fig 10, i believe that here you mean CBC2020 (pmiles, smiles etc)]}parsec models that have bigger equivalent width at younger ages than pyPopStar.

%Regarding Pa2 and Pa3 lines, pyPopStar models have stronger Paschen lines than all the empirical models, i.e, MaStar and MILES ( with both IMFs at all times). It seems that the reason behind this disagreement may be the different resolution of pyPopStar and MILES or MaStar.

%Last but not least, the Calcium Triplet (CaT) show two different behaviours: at intermediate ages and at old ages. At old ages ($\rm \tau > 1 \ Gyr$), the EW of pyPopStar models are very similar to the ones computed with the other models. At young and intermediate ages ($\rm 100-800 \ Myr$), pyPopStar models have higher EW than MILES and MaStar.


%Esta parte es para mostrar las ventajas de la HR. Hacer 
%1) TABLA de posibles a medir indices, UV, los de optico, CaT, alguno mas y sus continuos, recopilacion de otros hecho
%2) Mostrar perfiles de algunas lineas, variaciones con edad, con Z y con IMF
%3) Hacer tabla de los indices medidos Hecho
%4) Fig de algunos de esos indices a) ev. temporal para las 4 Z's en Kroupa b) ev temporal para 4 IMFs y una Z
\begin{table}
	\begin{center}
\caption{Ionisation potential of the species whose $Q$ is evaluated.}
\label{Table:5}
			\begin{tabular}{|c|c|}
				\hline
				Element & Wavelength \\
				\hline
				$\rm H \ I$ &  $ 911.8$\, \AA \\
				$\rm He \ I$ & $504.0$\, \AA \\
				$\rm O \ I$ & $ 353.3$\, \AA \\
				$\rm He \ II$ & $ 228.0$\, \AA \\
				\hline
			\end{tabular}
	\end{center}
\end{table}
